Globular Cluster Systems in Nearby Dwarf Galaxies: I. HST/ACS Observations and Dynamical Properties of Globular Clusters at Low Environmental Density

We investigate the old globular cluster (GC) population of 68 faint (Mv>-16 mag) dwarf galaxies located in the halo regions of nearby (<12 Mpc) loose galaxy groups and in the field environment based on archival HST/ACS images in F606W and F814W filters. The combined color distribution of 175 GC candidates peaks at (V-I)=0.96 +/- 0.07 mag and the GC luminosity function turnover for the entire sample is found at Mv,to = -7.6 +/- 0.11 mag, similar to the old metal-poor LMC GC population. Our data reveal a tentative trend of Mv,to becoming fainter from late-type to early-type galaxies. The luminosity and color distributions of GCs in dIrrs shows a lack of faint blue GCs. Our analysis reveals that this might reflect a relatively younger GC system than typically found in luminous early-type galaxies. If verified by spectroscopy this would suggest a later formation epoch of the first metal-poor star clusters in dwarf galaxies. We find several bright (massive) GCs which reside in the nuclear regions of their host galaxies. These nuclear clusters have similar luminosities and structural parameters as the peculiar Galactic clusters suspected of being the remnant nuclei of accreted dwarf galaxies, such as M54 and wCen. Except for these nuclear clusters, the distribution of GCs in dIrrs in the half-light radius vs. cluster mass plane is very similar to that of Galactic young halo clusters, which suggests comparable formation and dynamical evolution histories. A comparison with theoretical models of cluster disruption indicates that GCs in low-mass galaxies evolve dynamically as self-gravitating systems in a benign tidal environment.

==> Table2_short.tex <==
\begin{deluxetable}{p{1.8cm}p{3.9cm}p{1.9cm}p{1.8cm}p{1.6cm}p{.3cm}p{.3cm}p{.3cm}}
 \centering
\tablewidth{0pt}
%\rotate
\tablecaption{Globular cluster candidate properties (The full version of this table is available upon request).\label{table:GCCs}}
\tablehead{
\colhead{ID} & 
\colhead{RA,DEC\,(2000)} & 
\colhead{$M_V$} & 
\colhead{$(V-I)_0$} & 
\colhead{$r_{\rm h}$} & 
\colhead{$\epsilon$} & 
\colhead{r$_{\rm proj}$} & 
\colhead{r$_{\rm proj} / {\rm r}_{\rm eff}$} \\ 
\colhead{} & 
\colhead{[hh:mm:ss],[dd:mm:ss]} & 
\colhead{[mag]} & 
\colhead{[mag]} & 
\colhead{[pc]} & 
\colhead{} & 
\colhead{[kpc]} & 
\colhead{} \\
\colhead{(1)} & 
\colhead{(2)} & 
\colhead{(3)} & 
\colhead{(4)} & 
\colhead{(5)} & 
\colhead{(6)} & 
\colhead{(7)} & 
\colhead{(8)}
}

\startdata

	&	&	&	&	&	&	&	 \\
\multicolumn{8}{c}{dIrrs}\\
	&	&	&	&	&	&	&	 \\

E154-023-01  &  02:56:49.17  $-54:33:16.51$  &$   -4.78  \pm  0.06 $& $  1.045 \pm0.066 $   &$   2.27  \pm  0.30$ &  0.13  &  2.01 &   0.75 \\
IC1959-04    &  03:33:12.43  $-50:24:52.60$  &$   -9.83  \pm  0.05 $& $  0.968 \pm0.052 $   &$   2.92  \pm  0.20$ &  0.08  &  0.03 &   0.19 \\
N1311-01     &  03:20:20.05  $-52:10:14.95$  &$   -5.03  \pm  0.05 $& $  1.089 \pm0.055 $   &$   2.22  \pm  0.29$ &  0.20  &  3.39 &   2.95 \\
U685-01      &  01:07:26.18  $+16:40:56.84$  &$   -7.02  \pm  0.06 $& $  0.929 \pm0.062 $   &$   3.17  \pm  0.16$ &  0.00  &  1.28 &   1.88 \\
$\cdots$       &  $\cdots$                   &$   \cdots           $& $  \cdots         $   &$   \cdots         $ &  $\cdots$  &  $\cdots$ &   $\cdots$ \\

	&	&	&	&	&	&	&	 \\
\multicolumn{8}{c}{dSphs}\\
	&	&	&	&	&	&	&	 \\

IKN-01       &  10:08:07.14  $+68:23:36.65$  &$   -6.65  \pm  0.06 $& $  0.911 \pm0.079 $   &$   6.62  \pm  0.29$ &  0.13  &  0.40 &   -- \\
KKS55-01     &  13:22:12.41  $-42:45:11.76$  &$   -7.36  \pm  0.06 $& $  0.907 \pm0.078 $   &$   4.51  \pm  0.18$ &  0.11  &  1.48 &   4.75 \\
$\cdots$       &  $\cdots$                   &$   \cdots           $& $  \cdots         $   &$   \cdots         $ &  $\cdots$  &  $\cdots$ &   $\cdots$ \\

	&	&	&	&	&	&	&	 \\
\multicolumn{8}{c}{dEs}\\
	&	&	&	&	&	&	&	 \\

E269-66-05   &  13:13:11.79  $-44:53:09.79$  &$   -7.18  \pm  0.06 $& $  0.873 \pm0.078 $   &$   4.77  \pm  0.19$ &  0.16  &  0.63 &   1.03 \\
U7369-23     &  12:19:36.34  $+29:53:12.58$  &$   -6.68  \pm  0.07 $& $  0.848 \pm0.104 $   &$   1.35  \pm  0.42$ &  0.20  &  1.88 &   1.31 \\
$\cdots$       &  $\cdots$                   &$   \cdots           $& $  \cdots         $   &$   \cdots         $ &  $\cdots$  &  $\cdots$ &   $\cdots$ \\

	&	&	&	&	&	&	&	 \\
\multicolumn{8}{c}{Sms}\\
	&	&	&	&	&	&	&	 \\

E137-18-03   &  16:21:00.44  $-60:29:10.65$  &$   -7.15  \pm  0.07 $& $  1.143 \pm0.090 $   &$   3.11  \pm  0.21$ &  0.18  &  0.29 &   0.14 \\
E274-01-02   &  15:14:12.16  $-46:48:39.53$  &$   -7.78  \pm  0.06 $& $  0.864 \pm0.077 $   &$   3.97  \pm  0.17$ &  0.04  &  0.48 &   0.26 \\
N247-01      &  00:47:09.72  $-20:37:40.25$  &$   -7.42  \pm  0.06 $& $  0.859 \pm0.078 $   &$  16.02  \pm  0.28$ &  0.05  &  1.75 &   0.31 \\
N4605-08     &  12:40:13.58  $+61:35:12.72$  &$   -6.34  \pm  0.07 $& $  0.979 \pm0.091 $   &$  13.63  \pm  0.29$ &  0.16  &  3.43 &   1.26 \\
$\cdots$       &  $\cdots$                   &$   \cdots           $& $  \cdots         $   &$   \cdots         $ &  $\cdots$  &  $\cdots$ &   $\cdots$ \\

\enddata	
\end{deluxetable}

